A Dialogue Robot System to Improve Credibility in Sightseeing Spot Recommendations

Various studies have been conducted on human-supporting robot systems. These systems have been put to practical use over the years and are now seen in our daily lives. In particular, robots communicating smoothly with people are expected to play an active role in customer service and guidance. In this case, it is essential to determine whether the customer is satisfied with the dialog robot or not. However, it is not easy to satisfy all of the customer's requests due to the diversity of the customer's speech. In this study, we developed a dialog mechanism that prevents dialog breakdowns and keeps the customer satisfied by providing multiple scenarios for the robot to take control of the dialog. We tested it in a travel destination recommendation task at a travel agency.

==> tex/022-databases.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\hsize]{fig/CISRobot.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}



\begin{comment}

\end{comment}
